Search for long-lived heavy charged particles using a ring imaging Cherenkov technique at LHCb

A search is performed for heavy long-lived charged particles using 3.0 fb$^{-1}$ of pp collisions collected at $\sqrt{s}$= 7 and 8 TeV with the LHCb detector. The search is mainly based on the response of the ring imaging Cherenkovdetectors to distinguish the heavy, slow-moving particles from muons. No evidence is found for the production of such long-lived states. The results are expressed as limits on the Drell-Yan production of pairs of long-lived particles, with both particles in the LHCb pseudorapidity acceptance, $1.8 < \eta < 4.9$. The mass-dependent cross-section upper limits are in the range 2-4 fb (at 95\% CL) for masses between 124 and 309 GeV/c$^2$.

==> title-abstract.tex <==
  Search for  long-lived heavy charged particles using a
  ring imaging Cherenkov technique at LHCb


  \begin{abstract}
\noindent
A search is performed for heavy long-lived charged particles
using 3.0 fb$^{-1}$ of proton-proton collisions collected at $\sqrt{s}$= 7 and 8 TeV with the LHCb detector.
The search is mainly based on the response of the ring imaging Cherenkov
detectors to distinguish
the heavy, slow-moving particles from muons.
No evidence is found for the production of such long-lived states. 
The results are expressed as limits on the Drell-Yan production of pairs
of long-lived particles, with both particles in the LHCb pseudorapidity
acceptance, $1.8 < \eta < 4.9$.
The mass-dependent cross-section upper limits are in
the range 2--4~fb (at 95\% CL)
for masses between 124 and 309 GeV/c$^2$.

\end{abstract}

